Modeling and Selection of Interdependent Software Requirements using Fuzzy Graphs

Software requirement selection is to find an optimal set of requirements that gives the highest value for a release of software while keeping the cost within the budget. However, value-related dependencies among software requirements may impact the value of an optimal set. Moreover, value-related dependencies can be of varying strengths. Hence, it is important to consider both the existence and the strengths of value-related dependencies during a requirement selection. The existing selection models however, either assume that software requirements are independent or they ignore strengths of requirement dependencies. This paper presents a cost-value optimization model that considers the impacts of value-related requirement dependencies on the value of selected requirements (optimal set). We have exploited algebraic structure of fuzzy graphs for modeling value-related requirement dependencies and their strengths. Validity and practicality of the work are verified through carrying out several simulations and studying a real world software project.

==> notes.tex <==
Integer Linear Programming~\cite{ben_tal_lectures_2001}~\cite{golfarelli_multi_sprint_2013},~\cite{van_den_akker_flexible_2005}
 
Therefore, requirement selection is essentially a binary knapsack problem~\cite{harman_exact_2014},~\cite{zhang_multi_objective_2007},~\cite{carlshamre_release_2002},~\cite{lust_multiobjective_2012}.

future work: investigating the real distribution of interdependencies.
negative dependencies
compromise
other distributions can be used

multiple release
considering cost

%while maintaining negative value-related interdependencies will depreciates the overall value of optimal set. Nonetheless, none of the existing selection techniques have care for negative value-related inteSDPependencies. Nevertheless, for the sake of simplicity, we only focus on positive value-related interdependencies

%Example~\ref{ex_neg_dep} and Example~\ref{ex_pos_dep} provide examples of negative value-related dependencies~\cite{carlshamre_release_2002} and positive value-related dependencies~\cite{dahlstedt_requirements_2005} respectively. 

%\begin{exmp}
%\label{ex_neg_dep}
%A detailed online manual may decrease the (customer) value of a printed manual. 
%\end{exmp}

1) introduction
related work

2) By overall value, we mean perceived customer value. If all requirements are independent, they are same but.
3) More describe equation 3
4) Third, When requirements are highly interdependent, there would be only one collection of requirements
which is in fact the whole set of requirements. In such cases, this model will be degraded to the basic BKP
formula in Equation (1) as the whole set of requirements can never be realized (otherwise selection would not be
of any interest). 
5) Prototype


6) Refer this to Fig ? : For interdependency levels of greater than $0.25$ (in both RAN and PMR datasets) almost no value ($V_{ac/ov}$) was achieved by employing $BKP_G{pc}$ model unless budget was available

kukreja_value_based_2013


The results of our experiments showed that the \textit{accumulated value} of selected requirements can not properly measure the \textit{customer value} of optimal set as it does not consider the impacts of interdependent requirements on each other's values. However, this does not necessarily suggest that \textit{accumulated value} is not important to a selection process and can hereby be neglected. In fact, further research is required to investigate more useful applications of \textit{accumulated value}. Furthermore, the results of our experiments suggest that maximizing \textit{accumulated value} and maximizing \textit{overall value}, can be conflicting objectives. Therefore, a trade-off~\cite{marler_survey_2004,ben_tal_lectures_2001,ruhe_trade_2003} might be required to be made between these two objectives when both of them need to be considered. This can be another interesting trend for the future work.  

In addition, the same way as \textit{BKP} and \textit{BKP-PC} models, the \textit{GORS} model also does not consider the impact of requirements on each other's cost. In this way, the total cost of optimal set is calculated through aggregating the cost of selected requirements. However, requirements can impact each others cost~\cite{dahlstedt_requirements_2005,carlshamre_release_2002}. Therefore, another work is required to consider cost-related interdependencies along with the value-related interdependencies during the selection process. 

Last but not least, requirement selection is inherently a NP-hard problem~\cite{harman_exact_2014,li_integrated_2010,ruhe_art_2005,van_den_akker_flexible_2005,Martello_BKP_1990} as it involves computing the costs and values of all subsets of requirements. As such, any requirement selection model that finds the optimal set of requirements has a running time exponential to the number of the requirements~\cite{ben_tal_lectures_2001}. This is also the case for~\textit{GORS} model as well as the \textit{BKP} and \textit{BKP-PC} models. Although heuristics~\cite{boschetti_lagrangian_2014,leung_handbook_2004} and approximation~\cite{ruzika_approximation_2005} techniques have been proposed to reduce the complexity of requirement selection models, they do not guarantee finding optimal solutions~\cite{ruzika_approximation_2005}.





==> simulation_discussion.tex <==
\subsection{Remarks}
\label{sec_discussion}

\subsection{Remarks}
\label{sec_discussion}

The results of our simulation studies as well as a case study of a real-world software project have both consistently shown that: (a) the \textit{GORS} model can properly capture the strengths of dependency relations among requirements during selection process while mitigating the \textit{SDP}, (b) the \textit{GORS} model always maximizes the \textit{overall value} of the selected requirements, and (c) maximizing the overall and the accumulated values of an optimal set can be conflicting objectives~\cite{korte_combinatorial_2006} as maximizing one may depreciate the other.Therefore, a trade-off~\cite{marler_survey_2004,ben_tal_lectures_2001,ruhe_trade_2003} might be required to be made between these two objectives when both of them need to be considered. This can be another interesting trend for the future work.  

There are two major limitations to the present study as follows. First, identification of requirement dependencies and finding the strengths of those dependencies is a complex task when requirements are of large magnitude. There have been several techniques proposed in the literature~\cite{carlshamre_industrial_2001} to reduce that complexity. Nonetheless, dependency identification still remains a challenge to the software practitioners~\cite{carlshamre_industrial_2001}. Second, requirement selection in general is inherently a NP-hardproblem~\cite{harman_exact_2014,li_integrated_2010,ruhe_art_2005,van_den_akker_flexible_2005,Martello_BKP_1990}. 

As such, any requirement selection model that finds the optimal set of requirements has a running time exponential to the number of the requirements~\cite{ben_tal_lectures_2001}. This is also the case for~\textit{GORS} model as well as the \textit{BKP} and \textit{BKP-PC} models. Although heuristics~\cite{boschetti_lagrangian_2014,leung_handbook_2004} and approximation~\cite{ruzika_approximation_2005} techniques have been proposed to reduce the complexity of requirement selection models, they do not guarantee finding optimal solutions~\cite{ruzika_approximation_2005}. 



On the other hand, is inherently a NP-hardproblem~\cite{harman_exact_2014,li_integrated_2010,ruhe_art_2005,van_den_akker_flexible_2005,Martello_BKP_1990} and on the other hand, identification of requirement dependencies and finding the strengths of those dependencies could become a tedious task for larger number of requirements. Although there are several techniques proposed in the literature~\cite{carlshamre_industrial_2001} to reduce the complexity of dependency identification, this still remains a challenge to the software practitioners. 

As such, any requirement selection model that finds the optimal set of requirements has a running time exponential to the number of the requirements~\cite{ben_tal_lectures_2001}. This is also the case for~\textit{GORS} model as well as the \textit{BKP} and \textit{BKP-PC} models. Although heuristics~\cite{boschetti_lagrangian_2014,leung_handbook_2004} and approximation~\cite{ruzika_approximation_2005} techniques have been proposed to reduce the complexity of requirement selection models, they do not guarantee finding optimal solutions~\cite{ruzika_approximation_2005}. 



==> validation_simulation.tex <==
\subsection{Experimental Simulations}
\label{sec_simulation}

% prototype
% simulation
% Applicablity
This section presents the design and the results of our experimental simulations. 

==> validation_simulation_design.tex <==
\subsubsection{Experimental Design}%\textcolor{red}{(Is it worth including screenshots of your simulation user interface?)}}
\label{simulation_design}

We have compared the performance of the \textit{DARS} model against those of the existing selection models (namely \textit{BKP} and \textit{BKP-PC} models) through conducting several experiments on requirements from two distinct requirement sets. These requirement sets are taken from the following projects: Ericssons Radio Access Network (RAN) and the Performance Management Traffic Recording (PMR). The RAN project contains $14$ requirements identified by \textit{Ericsson Radio Systems} for a system that would give managers information about mobile telephony system operation. The PMR project contains $11$ requirements for recording and analyzing mobile telecommunications traffic~\cite{Karlsson_1996,karlsson_optimizing_1997,jung_optimizing_1998}. The values and costs of the requirements from RAN and PMR are listed in Table~\ref{table_data}.
%-----------------------------------------------
\begin{table}[!h]
\renewcommand{\arraystretch}{1.3}
%\extrarowheight as needed to properly center the text within the cells
\caption{Values and Costs of Requirements for the Experimental Datasets (RAN and PMR)}
\label{table_data}
\centering
\input{tables/table_data}
\end{table}
%-----------------------------------------------
\begin{figure}[h!]
\centering
\centerline{\hspace{-0.5em}\includegraphics[scale=0.7]{figs/fig_experiment.pdf}}
\vspace{-1em}
\caption{The experimental process}
\label{fig_experiment}
\end{figure}
%-----------------------------------------------

To the best of our knowledge, none of the existing requirement datasets has captured the strengths of dependency relations. As such, the distribution of dependency strengths is unknown and we have to rely on simulations. Simulation has been widely used for the purpose of evaluation in system analysis, operations research, and management science~\cite{Law_1997_SMA}. Chen et al.~\cite{li_integrated_2010} proposed simulating requirement interdependencies for analyzing the performance of requirement selection models. Other studies~\cite{wang_simulation_2012,cai_evolutionary_2012} have also simulated requirement dependencies. In a \textit{VDG}, strengths of value dependencies belong to the range of $[0,1]$. Therefore, we employed the \textit{nextDouble()} Method of the \textit{Random} Class in Java~\cite{java_random} to generate dependency strengths with a uniform distribution, which helps evaluate the performance of selection models for different levels of value dependencies among requirements. 

%-----------------------------------------------------------------------------
\begin{figure*}[!h]
\centering
\includegraphics[scale=0.8]{figs/demo}
    \caption{A Snapshot of Simulation User Interface}
    \label{fig_demo}
\vspace{0.2em}
\end{figure*}
%-----------------------------------------------------------------------------


Our experimental process is illustrated by Figure~\ref{fig_experiment}. The process starts with reading a requirements dataset. It then generates random numbers to specify the strengths of explicit dependency relations (edges of the graph) among all the requirements and construct the \textit{VDG} of the dataset as such. After that, it specifies a range of budget figures (for example. {1,2, ..., 120}) to examine the performance of the selection models in the presence of different budget constraints. At the end of each experiment cycle, an optimal set of requirements, together with its \textit{accumulated value} and \textit{overall value}, will be derived by each of the selection models. The experiment will be repeated for different levels of value dependencies (VDLs) (specified by Equation (\ref{Eq_loi})) and different levels of negative value dependencies (NVDLs) (specified by Equation (\ref{Eq_lonvd})) among the requirements of a dataset. A screen shot of our simulation user interface is given by Figure \ref{fig_demo}.

As discussed in Section \ref{sec_related}, some of the existing selection techniques~\cite{van_den_akker_flexible_2005, li_integrated_2010, sagrado_multi_objective_2013, Zhang_RIM_2013} rely on pair-wise comparisons among interdependent requirements to estimate their increased/decreased values. In these techniques stakeholders of the projects directly estimate the amount of increased/decreased values rather than considering the strengths of dependency relations. Therefore, the correlation between strengths of dependency relations and increased/decreased values are not specified in these techniques. Furthermore, implicit dependency relations are also not factored. For these reasons, we have not simulated these models in the present work.  
%Also we have employed ACME-Media dataset which is studied in the context of release panning~\cite{smith_becoming_2009}. For each experiment, a distinct set of random numbers are generated and assigned to the the strengths of dependency relations among requirements. Each experiment is repeated by different sets of random numbers to ensure the precision of outcomes.  

%-----------------------------------------------------------------------------------
\begin{figure*}
	\begin{center}
		\includegraphics[scale=0.8]{figs/fig_membership}
	\end{center}
	\caption{Membership function of ?}
	\label{fig_membership}
\end{figure*}
%-----------------------------------------------------------------------------------

==> validation_simulation_discussion.tex <==
\subsubsection{Limitations }
\label{sec_limitations}

Requirement selection is inherently a NP-hard problem~\cite{harman_exact_2014,li_integrated_2010,ruhe_art_2005,van_den_akker_flexible_2005,Martello_BKP_1990}. Nonetheles,  As such, any requirement selection model that finds the optimal set of requirements has a running time exponential to the number of the requirements~\cite{ben_tal_lectures_2001}. This is also the case for~\textit{GORS} model as well as the \textit{BKP} and \textit{BKP-PC} models. Although heuristics~\cite{boschetti_lagrangian_2014,leung_handbook_2004} and approximation~\cite{ruzika_approximation_2005} techniques have been proposed to reduce the complexity of requirement selection models, they do not guarantee finding optimal solutions~\cite{ruzika_approximation_2005}. 



==> validation_simulation_result.tex <==
\subsubsection{Experimental Results}
\label{sec_simulation_result}

We simulated the selection models of \textit{BKP}, \textit{BKP-PC}, and \textit{GORS} on requirements of RAN and PMR datasets. Our experiments were repeated to evaluate the efficiency of those selection models for different budgets and different levels of positive/negative value dependencies among the requirements. At the end of each simulation, three different optimal sets were generated by the three selection models. Figure~\ref{fig_result_0}, Figure~\ref{fig_result_1}, and Figure~\ref{fig_result_0.5}  show the results of our experiments for three different levels of negative value dependencies. The $x$ and $y$ axes show the available budget ($Budget \in \{0,1,...,120\}$) and the value dependency level ($VDL \in \{0,0.1,...,1\}$) in the \textit{VDG} of the dataset respectively. The $z$ axis shows the percentage of achieved accumulated/overall value of the optimal set, which is the ratio of $AV$ or $OV$ to the total value of the identified requirements expressed as a fraction of $100$. In all of the experiments, the \textit{BKP} model has achieved the maximal \textit{accumulated value} while the \textit{GORS} model has achieved the maximal \textit{overall value}. None of these models can maximize both $AV$ and $OV$ simultaneously, which indicates that maximizing $AV$ and $OV$ can be conflicting objectives as maximizing one may depreciate the other. 

\begin{figure*}
\begin{center}
\hspace{0em}	
\subfigure[Accumulated Value of RAN]{%
\label{fig:first}
\includegraphics[scale=0.55]{figs/result/ran-0-av}
}%
\subfigure[Accumulated Value of PMR]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/pmr-0-av}
}\\ %  ------- End of the first row ----------------------%
\subfigure[Overall Value of RAN]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/ran-0-ov}
}%
\subfigure[Overall Value of PMR]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/pmr-0-ov}
}
\end{center}
\caption{%
Accumulated and Overall Values of RAN and PMR for NVDL = 0.0
}%
\label{fig_result_0}
\end{figure*}
%-----------------------------------------------------------------------------------

Figures~\ref{fig_result_0},~\ref{fig_result_1}, and~\ref{fig_result_0.5} show that the efficiency of \textit{BKP-PC} model is severely impacted by the \textit{SDP} condition. In other words, the \textit{BKP-PC} model has generated the lowest $AV$ and $OV$ unless in the presence of a sufficient budget (that is $Budget \to 110$) and/or a negligible level of positive/negative value dependencies among the requirements (that is $VDL \to 0$). When all of the value dependencies are positive (that is NVDL=0) for $VDL > 0.25$ in both RAN and PMR datasets, almost no $AV$ or $OV$ was achieved by employing the \textit{BKP-PC} model unless budget was available for all of the requirements (for the example of the RAN dataset, $Budget=\displaystyle \sum_{i=1}^{14} c_i = 99$). In contrast, as shown by Figure \ref{fig_result_1}, when all of the value dependencies are negative (that is NVDL=1), the \textit{BKP-PC} model is less impacted by the adverse influence of $SDP$ because individual requirements can always be implemented independently when no other requirement is selected with them. For other cases of $NVDL$, as shown in Figure \ref{fig_result_0.5}, the impact of \textit{SDP} on the performance of the \textit{BKP-PC} model is between that of $NVDL=1$ and that of $NVDL=0$. 


\begin{figure*}
\begin{center}
\hspace{0em}	
\subfigure[Accumulated Value of RAN]{%
\label{fig:first}
\includegraphics[scale=0.55]{figs/result/ran-1-av}
}%
\subfigure[Accumulated Value of PMR]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/pmr-1-av}
}\\ %  ------- End of the first row ----------------------%
\subfigure[Overall Value of RAN]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/ran-1-ov}
}%
\subfigure[Overall Value of PMR]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/pmr-1-ov}
}
\end{center}
\caption{%
Accumulated and Overall Values of RAN and PMR for NVDL = 1.0
}%
\label{fig_result_1}
\end{figure*}

Figures~\ref{fig_result_0}, ~\ref{fig_result_1}, and ~\ref{fig_result_0.5} also show that the \textit{GORS} model has mitigated the impact of \textit{SDP} through considering the strengths of dependency relations among the requirements. The \textit{BKP} model however is not subject to \textit{SDP} as it completely ignores dependency relations among the requirements. The simulation results further show that all the selection models give the same amount of overall value when requirements are mutually independent, which however is unlikely to happen in real-world projects~\cite{carlshamre_industrial_2001}.
%-----------------------------------------------------------------------------------
\begin{figure*}
\begin{center}
\hspace{0em}	
\subfigure[Accumulated Value of RAN]{%
\label{fig:first}
\includegraphics[scale=0.55]{figs/result/ran-5-av}
}%
\subfigure[Accumulated Value of PMR]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/pmr-5-av}
}\\ %  ------- End of the first row ----------------------%
\subfigure[Overall Value of RAN]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/ran-5-ov}
}%
\subfigure[Overall Value of PMR]{%
\label{fig:second}
\includegraphics[scale=0.55]{figs/result/pmr-5-ov}
}
\end{center}
\caption{%
Accumulated and Overall Values of RAN and PMR for NVDL = 0.5
}%
\label{fig_result_0.5}
\end{figure*}
%-----------------------------------------------------------------------------------

\vspace{2em}
Figures~\ref{fig_result_ran} and~\ref{fig_result_pmr} compare the $AV/OV$ of  RAN and PMR datasets achieved by the three selection models of \textit{BKP}, \textit{BKP-PC}, and \textit{GORS} for different levels of value dependencies among the requirements. For the case of $VDL=0.5$ and $NVDL=0.0$, all of the randomly generated value dependencies are positive, while $50\%$ of them have non-zero strengths. The horizontal axis shows the available budget, while the vertical axis shows the percentage of achieved $AV$ or $OV$. In all of the experiments and for all levels of value dependencies, it is observed that the achieved overall value is almost always less than the accumulated  expected values of selected requirements. This is due to the fact that the \textit{overall value} of the optimal set has factored in the influences of excluded positive and included negative value dependencies on the \textit{accumulated value} of the selected requirements. 

\begin{figure*}
\begin{center}
\subfigure[VDL = $0.5$, NVDL = $0$]{%
\label{fig:first}
\includegraphics[scale=0.6]{figs/result/x-ran-0-50}
}%
\subfigure[VDL = $0.1$, NVDL = $0$]{%
\label{fig:second}
\includegraphics[scale=0.6]{figs/result/x-ran-0-10}
}\\ %  ------- End of the first row ----------------------%
\subfigure[VDL = $0.5$, NVDL = $1$]{%
\label{fig:third}
\includegraphics[scale=0.6]{figs/result/x-ran-1-50}
}%
\subfigure[VDL = $0.1$, NVDL = $1$]{%
\label{fig:fourth}
\includegraphics[scale=0.6]{figs/result/x-ran-1-10}
}%
\end{center}
\caption{%
Sample simulation results for RAN dataset
}%
\label{fig_result_ran}
\end{figure*}

\vspace{1em}
It is also observed that the gap between $AV$ and $OV$ of an optimal set grows as the level of value dependencies increases. The reason is that increasing the level of value dependencies among the requirements will increase the chance for non-zero-strength positive/negative value dependencies to exist. In the case of the \textit{BKP-PC} model, the \textit{AV} and the \textit{OV} of selected requirements always remain the same. The reason is that \textit{BKP-PC} formulates all of the value dependencies as precedence constraints of BKP formula and consequently the optimal set can only include those requirements whose positive value dependencies are all included in the set and whose negative dependencies are all excluded from the set.

\begin{figure*}
\begin{center}
\subfigure[VDL = $0.5$, NVDL = $0$]{%
\label{fig:first}
\includegraphics[scale=0.6]{figs/result/x-pmr-0-50}
}%
\subfigure[VDL = $0.1$, NVDL = $0$]{%
\label{fig:second}
\includegraphics[scale=0.6]{figs/result/x-pmr-0-10}
}\\ %  ------- End of the first row ----------------------%
\subfigure[VDL = $0.5$, NVDL = $1$]{%
\label{fig:third}
\includegraphics[scale=0.6]{figs/result/x-pmr-1-50}
}%
\subfigure[VDL = $0.1$, NVDL = $1$]{%
\label{fig:fourth}
\includegraphics[scale=0.6]{figs/result/x-pmr-1-10}
}%
\end{center}
\caption{%
Sample simulation results for PMR dataset
}%
\label{fig_result_pmr}
\end{figure*}
 
%--------------------------------------------------------------------------------------------


